Learning Representations for Parameter-Free Retrieval in Continual Fine-Tuning of Pre-Trained Models

Continual learning (CL) aims to adapt models to new tasks sequentially while preserving performance on earlier tasks whose data are no longer available. Many state-of-the-art (SOTA) methods leverage a pre-trained backbone augmented with lightweight fine-tuning modules to balance representation adaptability and knowledge retention. However, retrieval-based methods often retrieve fine-tuning modules at inference via continually learned retrieval functions that are themselves vulnerable to catastrophic forgetting. Alternatively, retrieval-free methods learn prediction mechanisms over a fixed pre-trained or pre-tuned representation space, avoiding forgetting induced by representation updates at the cost of adaptability. To overcome, we develop a novel CL framework that enables parameter-free retrieval by exploiting the distributional structures of task-adaptive representations. Our key insight is fine-tuning modules can be learned not only to acquire task-specific knowledge but also to induce representations that facilitate their own retrieval. Specifically, each fine-tuning module is paired with a compact statistical signature of its induced embedding distribution, enabling likelihood-based retrieval without continually updating a shared retriever. We theoretically characterize the conditions for accurate retrieval, showing that the per-input retrieval error decreases exponentially with representation separation, while the error of retrieving modules for single-task batches decreases exponentially with batch size under suitable conditions. Guided by this analysis, we develop a continual fine-tuning method that promotes representation distinguishability while facilitating cross-task knowledge transfer. Across class-incremental benchmarks, our approach achieves SOTA classification accuracy and the lowest average forgetting, while attaining highly competitive batch-wise retrieval accuracy.

==> contents/methods..tex <==
\section{Adaptive Knowledge Transfer and Parameter-Free Task-Retrieval
}\label{sec:adaptiveFT}
\vspace{-1mm}
\begin{figure}
    \centering
    \includegraphics[width=0.97\linewidth]{images/diagram.png}
    \caption{The overall workflow of the \textsc{Proteus} framework. {\bf A:} We optimize a LoRA unit for each task as a combination of previous tuning directions and new orthogonal components to capture task-specific information (Section~\ref{componnent1}). {\bf B:} We build a database of values (past update directions) and multi-keys (GMM parameters fit to each task embedding distribution). At test time, this database is used to retrieve most informative past updates per test input (Section~\ref{component3}). {\bf C:} We perform parameter-free prediction using linear discriminant analysis (Section~\ref{component3}).}
    \label{fig:Workflow SOLAR}
    \vspace{-5mm}
\end{figure}
\vspace{-2mm}
To address these limitations, we first note that each rank-$r$ LoRA update is equivalently written as a composition of rank-$1$ matrices, i.e., $\Delta\boldsymbol{\omega} \ \triangleq \ \boldsymbol{BA}^{\top}=\sum_{i=1}^r \boldsymbol{\phi}_i$, where each matrix $\boldsymbol{\phi}_i \triangleq \boldsymbol{B}_i\boldsymbol{A}_i^{\top}$ can be viewed as a \textit{tuning direction} pertaining to a task observed by the CL model. As new tasks continually emerge during training, re-learning these tuning directions from scratch without considering past updates will lead to poor distinction between task-specific representations, and hence poor retrieval of relevant knowledge at test time. To avoid this, we explicitly incorporate  constraints into LoRA-based fine-tuning that enforce orthogonality among the tuning directions of different tasks. This separation allows the model to focus on learning new, meaningful update directions whilst flexibly utilizing past updates whenever applicable. Indeed, our ablation studies show that these orthogonal components enhance the separability of input embeddings generated by different tasks' fine-tuning modules (Section~\ref{sec:ablation}). 

More interestingly, we show that these specialized tuning directions can be leveraged as signatures for \emph{task archetypes} during training, thus enabling \emph{parameter-free retrieval} and prediction during test time. In particular, the learned directions that emerge during the training phase are compiled into a database of keys and values that are used for identification of new tasks. Each task's key is defined by a mixture of probabilistic models learned from its induced input embeddings, whereas the value contains the corresponding task's fine-tuning module. During inference, each test input is matched to the mixture component (across all tasks) with the highest likelihood, enabling parameter-free retrieval and prediction (Section~\ref{component3}). The overview of our Proteus framework is illustrated in Fig.~\ref{fig:Workflow SOLAR}; we further describe in detail its synergistic components in the remainder of this section.

\subsection{Adaptive Knowledge Transfer and Discovery} \label{componnent1}
{\bf Knowledge Representation.}~Let $\boldsymbol{\phi}_{\tau,i}$ denote the $i^{\text{th}}$ new tuning direction for any task $\tau$. We note that each tuning direction $\boldsymbol{\phi}_{\tau,i}$ represents a rank-1 update, and is parameterized as an outer product of two vectors in $\boldsymbol{b}_{\tau,i} \in \mathbb{R}^p$ and $\boldsymbol{a}_{\tau, i} \in \mathbb{R}^q$.~For each new task $D_{k+1}$, we freeze old tuning directions, i.e., $\{\boldsymbol{\phi}_{\tau,i} \mid 1 \leq \tau \leq k$, $1 \leq i \leq r$\},
and subsequently represent its low-rank adaptation $\Delta\boldsymbol{\omega}_{k+1}$ as a (learnable) linear combination of old (frozen) and $r$ new tuning directions $\{\boldsymbol{\phi}_{k+1,i}\}_{i=1}^r$. 
 That is:
\vspace{-1mm}
\begin{eqnarray}
\hspace{-20.5mm}\Delta\boldsymbol{\omega}_{k+1} &\triangleq& \sum_{\tau=1}^k \sum_{i=1}^r s_{\tau,i} \boldsymbol{\phi}_{\tau,i} \ \ +\ \  \sum_{i=1}^r 
\boldsymbol{\phi}_{k+1, i}
\ \ = \ \ \sum_{\tau=1}^k \boldsymbol{B}_\tau\boldsymbol{S}_\tau\boldsymbol{A}^\top_\tau \ + \ \boldsymbol{B}_{k+1}\boldsymbol{A}^\top_{k+1} \ ,
\label{eq:9}
\end{eqnarray}
where $\boldsymbol{A}_\tau \triangleq [\boldsymbol{a}_{\tau,1}, \ldots, \boldsymbol{a}_{\tau,r}]$, $\boldsymbol{B}_\tau \triangleq [\boldsymbol{b}_{\tau,1}, \ldots, \boldsymbol{b}_{\tau,r}]$, and $\boldsymbol{S}_\tau \triangleq \mathrm{diag}[s_{\tau,1}, s_{\tau,2}, \ldots, s_{\tau,r}]$ are diagonal matrices that contain learnable linear coefficients corresponding to old tuning directions. 

{\bf Transfer and Discovery Components.}~Center to this representation is (1) the {\em knowledge discovery} term $\boldsymbol{B}_{k+1}\boldsymbol{A}_{k+1}^\top$ which captures the combination of new tuning directions specific to task $k + 1$; and (2) the {\em knowledge transfer} terms $\boldsymbol{B}_\tau\boldsymbol{S}_\tau\boldsymbol{A}_\tau^\top$ which specifies the transfer from a previous task $\tau$ to task $k+1$, by mixing relevant tuning directions according to the (learnable) signals encoded in $\boldsymbol{S}_\tau$.


{\bf Integrating Knowledge to Transfer and Discover.}~Incorporating (frozen) prior tuning directions into the parameterization of $\Delta\boldsymbol{\omega}_{k+1}$ enables knowledge transfer from previous tasks to new task. On the other hand, new tuning directions will be trained to capture unique adaptation patterns that are not relevant to $D_1, D_2, \ldots, D_k$. To ensure these directions contribute genuinely novel information that are specific to $D_{k+1}$, they must be orthogonal to the existing ones. Otherwise, they would lie within the span of previously learned directions and offer no additional value to the model. This gives rise to a set of linear constraints  $\left\langle\Delta\boldsymbol{\omega}_{k+1}^\perp, \Delta\boldsymbol{\omega}_\tau^\perp\right\rangle = 0$\footnote{$\langle\boldsymbol{u},\boldsymbol{v}\rangle \triangleq\ \mathrm{vec}(\boldsymbol{u})^\top\mathrm{vec}(\boldsymbol{v})$.} for all $\tau \leq k$, where $\Delta\boldsymbol{\omega}_{\tau}^\perp\triangleq\boldsymbol{B}_\tau\boldsymbol{A}_\tau^\top$.

We further note that, without any constraint on the knowledge transfer condition, $\boldsymbol{S}_\tau$ could assign non-zero weight to many directions from many past tasks even if they are only weakly relevant. To mitigate this and promote selective transfer, we additionally impose both $\ell_1$ and $\ell_2$-norm penalties than $\boldsymbol{S}_\tau$, which respectively encourage sparsity and low magnitude of the transfer. This forces the model to rely on a small number of past directions, and prevents excessive reliance on any single task. Hence, the continual learning objective at task $k+1$ can be succinctly written as:
\begin{eqnarray}
\hspace{-24mm}&\underset{\Delta\boldsymbol{\omega}_{k+1}^\perp, \boldsymbol{S}}{\minimize}&
L\left(\boldsymbol{\omega}_o 
 +  \sum_{\tau=1}^k \boldsymbol{B}_\tau\boldsymbol{S}_\tau\boldsymbol{A}_\tau^\top +  \Delta\boldsymbol{\omega}_{k+1}^\perp\right) + 
 \lambda \Big( \alpha \cdot \left\|\boldsymbol{S}\right\|_1 + (1 - \alpha) \cdot \left\|\boldsymbol{S}\right\|_2 \Big) \nonumber \\
\hspace{-24mm}&\text{subject to}& \forall \tau \leq k : \big\langle\Delta\boldsymbol{\omega}_{k+1}^\perp, \Delta\boldsymbol{\omega}_\tau^\perp\big\rangle = 0 \ , \quad \text{where} \quad \boldsymbol{S} = \mathrm{blkdiag}[\boldsymbol{S}_1,\ldots, \boldsymbol{S}_k] \ .
\label{eq:15_only}
\end{eqnarray}
We also performed sensitivity analysis to demonstrate the relative importance of hyper-parameters $\lambda$ (see Section~\ref{sec:ablation}) and $\alpha$ (see Appendix~\ref{sec: alpha-lambda}), and further provide empirical verification that the optimized solutions $\Delta\boldsymbol{\omega}_{\tau}^\perp$  indeed meet the orthogonality constraint (see Appendix~\ref{sec:orthogonal}). The full LoRA updates $\Delta\boldsymbol{\omega}_\tau$ are added to a database of task-specific tuning directions, which will be queried during test time to support inference of unseen queries (see Section~\ref{component3}).
\begin{algorithm}[t]
   \caption{\textsc{Proteus} Training}
   \label{alg:training_algs}
\begin{algorithmic}[1]
   \State {\bfseries INPUT:} pre-trained backbone $h(\boldsymbol{x}; \boldsymbol{\omega}_o)$ and stream of $m$ datasets $D_1, D_2, \ldots, D_m$
   \State {\bfseries OUTPUT:} database $\mathrm{KB} = \{ \text{multi-key}=(\boldsymbol{\Lambda}^k_\ast, \boldsymbol{m}_\ast^k)_{k=1}^\kappa, \text{value} = \Delta\boldsymbol{\omega}_\ast\}$; statistics $\boldsymbol{G}_S$, $(\boldsymbol{e}(c))_c$
   \State initialize $\mathrm{KB} \ \leftarrow\ \emptyset$, $\boldsymbol{G}_S \leftarrow \boldsymbol{0}$, $\boldsymbol{e}_S(c) \leftarrow \boldsymbol{0} \ \forall c$
   \For{$\tau=1$ {\bfseries to} $m$}
    \State compute $\text{\bf value} \ =\ \Delta\boldsymbol{\omega}_\tau$ via solving Eq.~\eqref{eq:15_only}
    \State compute $\text{\bf multi-key}= (\boldsymbol{\Lambda}_\tau^k, \boldsymbol{m}_\tau^k)_{k=1}^\kappa$ via Eq.~\eqref{eq:18}
    \State update $\mathrm{KB} \ \leftarrow\ \mathrm{KB} \ +\ \{\text{\bf multi-key},\text{\bf value}\}$
 
    \For {$(\boldsymbol{x}, z) \sim D_\tau$} -- running-sum update derived from Eq.~\eqref{eq:22}
        \State $\boldsymbol{G}_S \leftarrow \boldsymbol{G}_S + \boldsymbol{h}_S(\boldsymbol{x})\boldsymbol{h}_S(\boldsymbol{x})^\top$ 
        \State $\boldsymbol{e}_S(z) \leftarrow \boldsymbol{e}_S(z) + m^{-1}|D_\tau|^{-1}\boldsymbol{h}_S(\boldsymbol{x})$ 
    \EndFor
   \EndFor
   \State {\bfseries return} $\mathrm{KB}$, $\boldsymbol{G}_S$, $(\boldsymbol{e}_S(c))_{c \ \in\  \mathrm{class}}$
\end{algorithmic}
\end{algorithm}
%\vspace{-5mm}

\subsection{Parameter-Free Retrieval and Prediction} \label{component3}
As previously outlined in Section~\ref{sec:problem}, a central challenge in LoRA-based CL is selecting and retrieving the most relevant combination of previously acquired knowledge (e.g., LoRA units) to enable zero-shot inference on unseen test inputs. To facilitate this retrieval step, we introduce the concept of \textit{retrieval signatures} --- statistical descriptors associated with each stored LoRA unit, which allow us to assess its similarity to a given test input. Specifically, we note that each optimized LoRA unit modifies the pre-trained model in a task-specific manner, leading to a distinct distribution of input embeddings that reflects the characteristics of its corresponding task, and serves as a basis to guide retrieval. For example, if an input's LoRA-augmented embedding is statistically similar to samples drawn from probed embedding distribution induced by that same LoRA unit, it likely belongs to that task's distribution. Consequently, the LoRA unit will likely generate a strong representation for accurate prediction. We formalize this intuition below.

\textbf{Parameter-Free Retrieval.} Let $\boldsymbol{x}$ be a test input, and $\boldsymbol{h}_k(\boldsymbol{x}) =h(\boldsymbol{x}; \boldsymbol{\omega}_o \ +\  \Delta\boldsymbol{\omega}_k)$ be its induced embedding under $\Delta \boldsymbol{\omega}_k$. A matching signature for $\Delta\boldsymbol{\omega}_k$ could be characterized by a probabilistic model that summarizes the LoRA-augmented embeddings for inputs from $D_k$. In particular, one simple approach is to view the observed input embeddings $\boldsymbol{h}_k(\boldsymbol{x})$ where $\boldsymbol{x} \sim D_k$ as samples from a Gaussian distribution whose parameters, e.g., its mean and covariance matrices, can be learned via Maximum Likelihood Estimation (MLE):
\begin{eqnarray}
\hspace{-2.5mm}
\left(\boldsymbol{m}_k, \boldsymbol{\Lambda}_k\right) 
\ =\ 
\argmin_{\boldsymbol{m},\boldsymbol{\Lambda}} \ \sum_{\boldsymbol{x} \in D_k} S_k(\boldsymbol{x}; \boldsymbol{m}, \boldsymbol{\Lambda})
\ \triangleq\  \argmin_{\boldsymbol{m},\boldsymbol{\Lambda}} \ \sum_{\boldsymbol{x} \in D_k} \left(\boldsymbol{h}_k(\boldsymbol{x}) - \boldsymbol{m}\right)^\top \boldsymbol{\Lambda}^{-1}\left(\boldsymbol{h}_k(\boldsymbol{x}) - \boldsymbol{m}\right) . \hspace{-5mm}
\label{eq:retrieval_gaussian}
\end{eqnarray}
In the above, the signature function $S_k(\boldsymbol{x}; \boldsymbol{m}, \boldsymbol{\Lambda})$ is given by the negative log Gaussian likelihood of $\boldsymbol{h}_k(\boldsymbol{x})$ with mean $\boldsymbol{m}$ and covariance $\boldsymbol{\Lambda}$. During test time, each test input $\boldsymbol{x}_\ast$ will be mapped to a training task via maximizing the same signature likelihood function, i.e., $k_\ast = \argmin_k S_k(\boldsymbol{x}_\ast)$. We note that the signature parameters are individually learned for each observed task after training, making the retrieval function parameter-free in the sense that it does not involve any parameters subject to forgetting during continual learning.

This however assumes a single representation pattern for each task, since the Gaussian distribution is unimodal. To generalize this framework, we instead learn a mixture of Gaussian components for the observed input embeddings. This is achieved via replacing the optimization task in Eq.~\eqref{eq:retrieval_gaussian} with
\vspace{-1mm}
\begin{eqnarray}
\hspace{-0.25mm}\minimize_{\boldsymbol{m}^{1:\kappa}, \boldsymbol{\Lambda}^{1:\kappa}, \{\zeta_{it}\}} \quad \sum_{t=1}^\kappa\sum_{i=1}^{|D|} \zeta_{it} \cdot S_k\Big(\boldsymbol{x}_i; \boldsymbol{m}^t, \boldsymbol{\Lambda}^t\Big) \quad \text{such that} \quad \zeta_{it} \in \{0, 1\} \quad \text{and} \quad \sum_{t=1}^\kappa \zeta_{it} = 1 \ . \label{eq:18}
\end{eqnarray}
This formulation imposes a \emph{multi-key signature} for the input embeddings under task $k$. To avoid fixing the number of components $\kappa$, we can further view the above as a clustering task and instead adopt a generalized non-parametric clustering scheme such as the Dirichlet Process for Gaussian Mixture Models (DP-GMMs)~\cite{teh2010dirichlet}, which automatically learns the best value for $\kappa$ in addition to the corresponding distribution parameters for each Gaussian component. During inference, each test input $\boldsymbol{x}_\ast$ is again matched to the training task with highest signature score, i.e.,
$(k_\ast, t_\ast) = \argmin_{k, t}  S_k^\tau\left(\boldsymbol{x}_\ast; \boldsymbol{m}_k^t, \boldsymbol{\Lambda}_k^t\right)$,
which retrieves the specific LoRA $\Delta\boldsymbol{\omega}_{k_\ast}$ in our database.

{\bf Parameter-Free Prediction.} In what follows, we will use the notations $\Delta\boldsymbol{\omega}_S(\boldsymbol{x}_\ast) = \boldsymbol{\omega}_{k_\ast}$ and $\boldsymbol{h}_S(\boldsymbol{x}_\ast) = h\left(\boldsymbol{x}_\ast; \boldsymbol{\omega}_o \ \ +\ \    \Delta\boldsymbol{\omega}_S(\boldsymbol{x}_\ast)\right)$ to indicate the retrieved LoRA unit for $\boldsymbol{x}_\ast$ and its corresponding LoRA-augmented embedding. Similar to RanPAC, we can again compute the necessary statistics (in running sum fashion, see Alg.~\ref{alg:training_algs}) for the parameter-free LDA prediction scheme,\vspace{-2mm}
\begin{eqnarray}
\hspace{-5mm}\boldsymbol{G}_S = \sum_{\tau=1}^m \sum_{\boldsymbol{x} \in D_\tau} \boldsymbol{h}_S\big(\boldsymbol{x}\big)\boldsymbol{h}_S\big(\boldsymbol{x}\big)^\top \quad \text{and} \quad
\boldsymbol{e}_S(c) = \frac{1}{m|D_\tau|}\sum_{\tau = 1}^m \sum_{(\boldsymbol{x},z) \in D_\tau}\boldsymbol{I}\big(z = c\big) \cdot \boldsymbol{h}_S\big(\boldsymbol{x}\big),\label{eq:22}
\end{eqnarray}

\vspace{-2mm}
which then induce the final parameter-free prediction: \vspace{-2mm}
\begin{eqnarray}
c_\ast &=& \argmax_c\ \  \boldsymbol{h}_S(\boldsymbol{x}_\ast)^\top \Big(\boldsymbol{G}_S + \gamma\boldsymbol{I}\Big)^{-1}\boldsymbol{e}_S(c) \ , \label{eq:23}    
\end{eqnarray}

\vspace{-2mm}
where $\gamma > 0$ is a user-specified noise level. This results in strong adaptation across tasks which lead to superior performance as consistently demonstrated across an extensive set of benchmark datasets (see Section~\ref{sec:main-results}). Finally, we give the pseudocode for the training of Proteus in Alg.~\ref{alg:training_algs}; the pseudocode for inference in Appendix~\ref{sec:inference-pseudocode}; their empirical memory consumption analysis in Fig.~\ref{fig:complexity}; and memory complexity in Appendix~\ref{sec: memory}.

{\bf Remark.} We note that despite using a similar prediction form as RanPAC~\cite{DBLP:conf/nips/McDonnellGPAH23}, the input embeddings used in both the prediction and sufficient statistic computation of $\boldsymbol{G}_S$ and $\boldsymbol{e}_S(c)$ are customized for each input via the parameter-free retrieval process in Eq.~\eqref{eq:18}. This is enabled by our earlier contribution on {\em parameter-free retrieval}.~Otherwise, the parameter-free prediction mechanism is adopted from RanPAC~\cite{DBLP:conf/nips/McDonnellGPAH23} and is not part of our contribution.\vspace{-2mm}




